The Emergence of the First Star-free Atomic Cooling Haloes in the Universe

Using the Renaissance suite of simulations we examine the emergence of pristine atomic cooling haloes that are both metal-free and star-free in the early Universe. The absence of metals prevents catastrophic cooling, suppresses fragmentation, and may allow for the formation of massive black hole seeds. Here we report on the abundance of pristine atomic cooling haloes found and on the specific physical conditions that allow for the formation of these direct-collapse-black-hole (DCBH) haloes. In total in our simulations we find that 79 DCBH haloes form before a redshift of 11.6. We find that the formation of pristine atomic haloes is driven by the rapid assembly of the atomic cooling haloes with mergers, both minor and/or major, prior to reaching the atomic cooling limit a requirement. However, the ability of assembling haloes to remain free of (external) metal enrichment is equally important and underlines the necessity of following the transport of metals in such simulations. The candidate DCBH hosting haloes we find, have been exposed to mean Lyman-Werner radiation fields of J$_{LW}$ $\sim$ 1 J$_{21}$ and typically lie at least 10 kpc (physical) from the nearest massive galaxy. Growth rates of the haloes reach values of greater than 10$^7$ M$_{\odot}$ per unit redshift, leading to significant dynamical heating and the suppression of efficient cooling until the halo crosses the atomic cooling threshold. Finally, we also find five synchronised halo candidates where pairs of pristine atomic cooling haloes emerge that are both spatially and temporally synchronised.

==> Makefile <==

USE_BIBTEX=yes
TEX=pdflatex
BIBTEX=bibtex
PDF=dvipdf
all: ha.pdf 


ha.pdf: ha.tex
	$(TEX) ha.tex $@
	$(TEX) ha.tex $@	
	$(BIBTEX) ha
	$(BIBTEX) ha
	$(TEX) ha.tex $@
	$(BIBTEX) ha
	$(TEX) ha.tex $@
	$(TEX) ha.tex $@
#$(PDF) ha.dvi
.PHONY : clean

clean:
	rm -f *.log *.aux *.out *.dvi *.blg *.toc *.lof *.lot *.tbx \
	 *.fgx *~ ha.pdf ha.ps *.bbl


